Analysis of a Bloom Filter Algorithm via the Supermarket Model

This paper deals with the problem of identifying elephants in the Internet Traffic. The aim is to analyze a new adaptive algorithm based on a Bloom Filter. This algorithm uses a so-called min-rule which can be described as in the supermarket model. This model consists of joining the shortest queue among d queues selected at random in a large number of m queues. In case of equality, one of the shortest queues is chosen at random. An analysis of a simplified model gives an insight of the error generated by the algorithm on the estimation of the number of the elephants. The main conclusion is that, as m gets large, there is a deterministic limit for the empirical distribution of the filter counters. Limit theorems are proved and the limit is identified. It depends on key parameters. The condition for the algorithm to perform well is discussed. Theoretical results are validated by experiments on a traffic trace from France Telecom and by simulations.

==> Intro.tex <==
\section{Introduction}
To be efficient, network traffic measurement methods have to be adapted to the actual traffic characteristics. 
Internet links are currently carrying a huge amount of data at a very high bit rate (40 Gb/s in OC-768). To analyze on-line this traffic, scalable algorithms are required. They have to operate fast, using a limited small memory. The traffic is mainly analyzed at the {\em flow} level. 
A flow is a sequence of packets defined by the classical 5tuple
composed of the source and destination addresses, the source and
destination port numbers together with the protocol type. Flows
statistics are very useful for traffic engineering and network
management. In particular, information about large flows (also called
elephants) is very interesting for many applications. Note that an
elephant is a flow with at least $K$ packets, where $K$ is in practice equal
to 20. Elephants are not numerous (around 5 to 20\% of the number of
flows), but they represent the main part (80-90 \%) of the traffic
volume in terms of packets. Elephants statistics can be exploited in
various fields such as attacks detection or accounting. In the
literature, some probabilistic algorithms have been developed to
estimate on-line the number of elephants in a dense traffic. In
\cite{Flajolet-1}, Flajolet analyzed the Adaptive Sampling algorithm
proposed by Wegman. This algorithm is based on a special sampling
method that provides a random set of the original flows. Some
characteristics on elephants (number, size distribution) can be
inferred from this sample. Some other algorithms (see \cite{Gandouet-1,Yousra}) based on sampling are designed to provide elephants statistics, but they seem to be designed to very specific flow size distribution or require an a priori knowledge of the total number of flows to recover the loss of information caused by the sampling. Moreover all these algorithms are not able to identify elephants, that is to give their addresses. Such information is particularly useful for attacks detection.

For that, Estan and Varghese \cite{Estan-1} propose an algorithm based on Bloom filters. This algorithm is quick enough and it uses a limited memory, but it is not adapted to traffic variations. It uses a fixed parameter which should be adjusted according to traffic intensity.
Azzana  in \cite{Azzana-1} then Chabchoub \etal~ \cite{Chabchoub:01}
propose an improvement for this algorithm by adding a refreshment
mechanism that depends on traffic variations. The principle of this
latter algorithm is the following. The filter is composed of $d$
stages. Each stage contains $m$ counters and is associated to a
hashing function. When a packet is received, its IP header is hashed
by the $d$ independent hashing functions and the corresponding counter
in each stage is incremented by one. When a counter reaches $K$ (the
smallest elephants size), the corresponding flow is considered as an
elephant. Due to the heavy Internet traffic, the filter needs to be
sometimes refreshed, otherwise all the counters will exceed the threshold
$K$, and then all the flows will be seen as elephants. The idea is to
decrease all counters by one every time the proportion of non null
counters reaches a given threshold $r$. In this way the refreshment
frequency of the filter depends closely on the actual traffic
intensity. Notice that the algorithm uses an improvement, the {\em
  min-rule}, also called {\em conservative update} in
\cite{Estan-1}. It consists in incrementing only the counters among
$d$ having the minimum value, for an arriving packet. Indeed, because
of collisions, the flow size is at most given by the smallest
associated counters. So the min-rule reduces the overestimation of
flow size. This algorithm  has been first presented in \cite{Azzana-1}. In \cite{Chabchoub:01}, a more complete version of the algorithm is developed. A new refreshment mechanism based on the average of counters values is added. In addition, the algorithm (under some modifications) is applied to attacks detection. These algorithms are validated using several traffic traces.  

 Chabchoub \etal~ present in \cite{Chabchoub:02} a theoretical
 analysis of the algorithm proposed by Azzana and described
 above. Their objective is to estimate the error generated by the
 algorithm on the estimation of number of elephants. The analytical study does not take into account the min-rule. 

In this paper, we focus on the analysis of the min-rule. For this purpose, the algorithm described above has been slightly modified. We consider now just one filter and two hashing functions ($d=2$). An arriving packet increments the smallest counter among the two associated counters. In case of equality, only one counter is incremented at random. In this way, every packet increments exactly one counter. A flow is declared as an elephant when its smallest associated counter reaches $C=K/d$. The same refreshment mechanism is maintained with a threshold $r$ of about $50\%$. The basic idea is that when the filter is not overloaded, in general, for each arriving packet of a given flow, one of the two counters will be incremented in an alternative way. It means that the two counters will have almost the same values and when the smallest one reaches $C$, the corresponding flow has a total size of about $K=dC$ packets ($C$ packets hitting  each counter). 

The advantage of this new algorithm is that each arriving packet
increments exactly one counter. In this case the way to increment the
counters is exactly, in a system of $m$ queues, the way a customer
joins the shortest queue among $d$ queues chosen at random, ties being
solved at random. This so-called {\em supermarket model} by Luczak and
McDiarmid \cite{Luczak-1,Luczak-3}, also known as  {\em load-balancing
model} with the choice, has been extensively studied in the literature
because of its numerous useful applications. In computer science, the
central result is stated in a pioneer paper by Azar \etal~
\cite{Azar-1} then Miztenmacher \cite{Mitzenmacher-1}, for a discrete time model when $n$ balls are
thrown into $n$ urns with the choice.  It is proved that, with
probability tending to $1$ as $n$ gets large, the maximum load of an
urn is $\log n/\log \log n+O(1)$ when $d=1$ and $\log \log n/\log d
+O(1)$ if $d\geq 2$. Luczak and McDiarmid, in  continuous time related
models with the choice, explore the concentration of the maximum queue
length (see \cite{Luczak-1}, \cite{Luczak-2}). But the model had also
already been studied in Vvedenskaya \etal~ \cite{Vvedenskaya-1},
Graham \cite{Graham-3} and others for mean-field limit theorems. In
\cite{Vvedenskaya-1}, a functional law of large numbers is stated: The
vector  of the tail proportions of  queues  converges in distribution
as $m$ tends to infinity  to the unique solution of a differential
system. The differential equation has a unique fixed point
$u^{\rho}(k)=\rho^{(d^k-1)/(d-1)}$ for a throughput $\rho$. It means
that, when $d\geq 2$, the tail probabilities of the queue length
decrease drastically.
In Vvedenskaya and Suhov \cite{Vvedenskaya-4},  variants of the
choice policy  and  general service time distributions are
investigated. Graham in \cite{Graham-3} proves the convergence of the invariant measures to some Dirac measure. In other words, when $m$ is large, the stationary vector of the proportions of queues with $k$ customers is essentially deterministic and given by this limit. 

The aim of this paper is to model the min-rule via the supermarket
model and to evaluate the performance of the new proposed
algorithm. In particular, we want to calculate the error generated by
the algorithm on the estimation of number of elephants. Notice that
this error is due to both false negatives (missed elephants) and false
positives (mice considered as elephants). Let us focus on false
positives. To be declared as an elephant, a mouse must be hashed to
one among counters greater than  $C$ after this operation. So the proportion of such counters is a good parameter to investigate in order to evaluate false positives. 

% Moreover, we will show that the number of packets between two refreshments is also a key parameter for the analysis of the algorithm.

The most part of the paper is the analysis of a simple model where the flows are mice of size one. It is relevant because most of the flows are mice so collisions between flows are mainly due to collisions between mice.
It turns out that the probability that a mouse is detected as an
elephant is bounded by the probability that a given counter is greater
than $C$ just before a refreshment time. Thus the problem reduces to
analyze the  behavior of the model at the refreshment times. Moreover
the transition phase is very short thus the study of the stationary
behavior is pertinent.

The key idea of the study is to use the Markovian framework in order
to rigorously establish limit theorems and analytical expressions in
the stationary regime. The main result is  that, as $m$ tends to
infinity, the evolution of the model is characterized by a dynamical
system which has at least one fixed point. When $d=1$, this fixed point is  unique and denoted by $\bar{w}$. In this paper, we conjecture its uniqueness when $d \geq 2$. The interpretation of
$\bar{w}$ as a key quantity in a supermarket model with deterministic
service times is discussed. Analytical expressions are given in
\cite{Chabchoub:02} for $d=1$, are more complicated to obtain here.  

An objective would be to prove the convergence of the invariant
measure of the Markov chain as $m$ tends to $+\infty$ to the Dirac
measure $\delta_{\bar{w}}$ at the fixed point $\bar{{w}}$. In
practice, such a result is completely crucial. If it is not true, if
the sequence of invariant measures do not converge, the system
oscillates with long periods of transition between different
configurations (metastability phenomenon). So even if the algorithm
performs well during a while, it can reach another state where it can give bad results. This question is partially addressed here. But the convergence of the invariant measures is conjectured, due to simulations of the algorithm where
such a phenomenon has not been observed. For such a result, a possible
technique is the existence of a Lyapounov function which both proves the convergence of the dynamical system to its unique fixed point $\bar{w}$ and the convergence of the sequence of invariant measures to $\delta_{\bar{w}}$. Such a function is exhibited in \cite{Chabchoub:02} for $d=1$ and $C=2$.

A simulation of the limit distribution $\bar{w}$ is done for a uniform
general mice size distribution. Experiments have two goals. First to compare the original version presented in \cite{Chabchoub:01} and the version of the algorithm introduced here. Second, the time between two refreshments is plotted. This quantity is  crucial for the trade-off between false positives and false negatives. The time to reach the stationary phase is discussed.

The organization of the paper is as follows: Section II presents the analytical results for  the simple model defined to study the question of false positives. Section III is devoted to experiments. Section IV gives a discussion of the way to choose the parameter $r$ in order to have an algorithm which performs well. 



==> finIntro.tex <==
The most part of the paper is the analysis of a simple model where the flows are mice of size one. It is relevant because most of the flows are mice so collisions between flows are mainly due to collisions between mice.
It turns out that the probability that a mouse is detected as an elephant is bounded by the probability that a given counter is greater than $C-1$ just before a refreshment time. Thus the problem reduces to analyze the stationary behavior of the model when the number of counters gets large. 

The key idea of the study is to use the Markovian framework in order to rigorously establish limit theorems and analytical expressions in the stationary regime. The main result is  that, as $m$ tends to infinity, the evolution of the model is characterized by a dynamical system which has a unique fixed point $\bar{w}$.The interpretation of $\ber{w}}$ as a key quantity in a supermarket model with deterministic service times is discussed. Analytical expressions, can be given for $d=1$, are complicated to obtain here.  

 A objective would be to prove the convergence of the invariant measure of the Markov chain as $m$ tends to $+\infty$ to the Dirac measure $\delta_{\bar{w}}$ at the fixed point $\bar{{w}}$. In practice, such a result is completely crucial. If it is not true, if the sequence of invariant measures do not converge, the system oscillates with long periods of transition between different configurations. So even if the algorithm preforms well, it can reach another state where it can give bad results. This question is partially adressed here. But the convergence of the invariant measures is conjectured, due to simulations of the algorithm where
such a phenomenon has not been observed. For such a result, a possible technique is the existence of a Lyapounov function which proves the convergence of the dynamical system to its unique fixed point $\bar{w}$ and the convergence of the sequence of invariant measures to $\delta{\bar{w}}$. Such a function is exhibited in \cite{Chabchoub-} for $d=1$ and $C=2$.

